Multi-stages attention Breast cancer classification based on nonlinear spiking neural P neurons with autapses

Breast cancer(BC) is a prevalent type of malignant tumor in women. Early diagnosis and treatment are vital for enhancing the patients' survival rate. Downsampling in deep networks may lead to loss of information, so for compensating the detail and edge information and allowing convolutional neural networks to pay more attention to seek the lesion region, we propose a multi-stages attention architecture based on NSNP neurons with autapses. First, unlike the single-scale attention acquisition methods of existing methods, we set up spatial attention acquisition at each feature map scale of the convolutional network to obtain an fusion global information on attention guidance. Then we introduce a new type of NSNP variants called NSNP neurons with autapses. Specifically, NSNP systems are modularized as feature encoders, recoding the features extracted from convolutional neural network as well as the fusion of attention information and preserve the key characteristic elements in feature maps. This ensures the retention of valuable data while gradually transforming high-dimensional complicated info into low-dimensional ones. The proposed method is evaluated on the public dataset BreakHis at various magnifications and classification tasks. It achieves a classification accuracy of 96.32% at all magnification cases, outperforming state-of-the-art methods. Ablation studies are also performed, verifying the proposed model's efficacy. The source code is available at XhuBobYoung/Breast-cancer-Classification.

==> table.tex <==
%将下面这一行放置到文章首部\usepackage那里
\usepackage{multirow}
%下方全是代码。分别是表一，表二，表三。ta1和ta2，ta3分别是他们的引用标签
%表一：
\begin{table}[]
\begin{tabular}{ccccccc}
\hline
Environments               & Gestures                                                             & \begin{tabular}[c]{@{}c@{}}No.of\\ User\end{tabular} & \begin{tabular}[c]{@{}c@{}}No.of\\ Locations\end{tabular} & \begin{tabular}[c]{@{}c@{}}No.of\\ Orientations\end{tabular} & \begin{tabular}[c]{@{}c@{}}No.of\\ collections\end{tabular} & \begin{tabular}[c]{@{}c@{}}No.of\\ Samples\end{tabular} \\ \hline
\multirow{2}{*}{Classroom} & 1.Push Pull                                                          & \multirow{2}{*}{9}                                   & \multirow{2}{*}{5}                                        & \multirow{2}{*}{5}                                           & \multirow{2}{*}{5}                                          & \multirow{2}{*}{10125}                                  \\
                           & 2.Sweep                                                              &                                                      &                                                           &                                                              &                                                             &                                                         \\
\multirow{2}{*}{Hall}      & 3.Clap                                                               & \multirow{2}{*}{4}                                   & \multirow{2}{*}{5}                                        & \multirow{2}{*}{5}                                           & \multirow{2}{*}{5}                                          & \multirow{2}{*}{2250}                                   \\
                           & 4.Slide                                                              &                                                      &                                                           &                                                              &                                                             &                                                         \\
\multirow{2}{*}{Office}    & \begin{tabular}[c]{@{}c@{}}5.Draw-O\\ (Horizontal)\end{tabular}      & \multirow{2}{*}{3}                                   & \multirow{2}{*}{5}                                        & \multirow{2}{*}{5}                                           & \multirow{2}{*}{5}                                          & \multirow{2}{*}{3000}                                   \\
                           & \begin{tabular}[c]{@{}c@{}}6.Draw-Zigzag\\ (Horizontal)\end{tabular} &                                                      &                                                           &                                                              &                                                             &                                                         \\ \hline
\end{tabular}
\caption{SAMPLE OF THE WIDAR DATASET USED FOR THE PRESENTATION}
\label{ta1}
\end{table}



%表二：
%引用直接在下文中替换“文献”填写
\begin{table}[]
\begin{tabular}{ccccc}
\hline
Method          & In-domain        & Cross-Location   & Cross-Orientation & Cross-Environment \\ \hline
Widar3.0  \cite{文献}      & 92.70\%          & 89.70\%          & 82.60\%           & 92.40\%           \\
DFGR            & 93.20\%          & 92.10\%          & 92.10\%           & 92.10\%           \\
WiHF with HuFuM & 93.92\%          & 90.32\%          & 79.14\%           & 89.67\%           \\
WiHF with HuFu  & 97.65\%          & 92.07\%          & 82.38\%           & -                 \\
WiGr            & 92.70\%          & 75.00\%          & 84.00\%           & 83.00\%           \\
WiGRUNT         & \textbf{99.71\%} & \textbf{96.62\%} & 93.85\%           & \textbf{93.73\%}  \\
Wi-Learner      & 93.20\%          & 91.40\%          & 86.50\%           & 74.20\%           \\
The Proposed    & 98.22\%          & 94.60\%          & \textbf{94.71\%}  & 91.79\%           \\ \hline
\end{tabular}
\caption{Sample of Wider dataset}
\label{ta2}
\end{table}

%表三：
\begin{table}[]
\begin{tabular}{cccccc}
\hline
Gesture\textbackslash{}Target Label & 1       & 2       & 3       & 4       & 5       \\ \hline
In-Domain                           & 98.22\% & 98.22\% & 98.22\% & 98.22\% & 98.22\% \\
Cross-Location                      & 94.56\% & 92.00\% & 93.78\% & 95.56\% & 97.11\% \\
Cross-orientation                   & 92.00\% & 97.00\% & 94.22\% & 95.33\% & 95.00\% \\
Cross-Environment                   & 86.03\% & 92.53\% & 96.80\% & -       & -       \\ \hline
\end{tabular}
\caption{Accuracy for the proposed SNN on wiadr3.0 dataset}
\end{table}
